An Empirical Analysis on Spatial Reasoning Capabilities of Large Multimodal Models

Large Multimodal Models (LMMs) have achieved strong performance across a range of vision and language tasks. However, their spatial reasoning capabilities are under-investigated. In this paper, we construct a novel VQA dataset, Spatial-MM, to comprehensively study LMMs' spatial understanding and reasoning capabilities. Our analyses on object-relationship and multi-hop reasoning reveal several important findings. Firstly, bounding boxes and scene graphs, even synthetic ones, can significantly enhance LMMs' spatial reasoning. Secondly, LMMs struggle more with questions posed from the human perspective than the camera perspective about the image. Thirdly, chain of thought (CoT) prompting does not improve model performance on complex multi-hop questions involving spatial relations. % Moreover, spatial reasoning steps are much less accurate than non-spatial ones across MLLMs. Lastly, our perturbation analysis on GQA-spatial reveals that LMMs are much stronger at basic object detection than complex spatial reasoning. We believe our benchmark dataset and in-depth analyses can spark further research on LMMs spatial reasoning. Spatial-MM benchmark is available at: https://github.com/FatemehShiri/Spatial-MM

==> figures/spatial-gqa-multi-hop.tex <==
\begin{figure}[ht]
    \centering
    \resizebox{.5\textwidth}{!}{
    \includegraphics{images/spatial-gqa-multi-hop.pdf}}
    \caption{Spatial-GQA-Multi-hop Question Generation Example. $q_1$ is a spatial-related question (indicated by words in green) filtered using format matching, and $q_2$ is a answer-related question (indicated by words in blue) searched using the answer $a_2$. ChatGPT replaced the $a_2$ in $q_1$ (indicated by words in orange), and kept the answer the same with $q_1$ (indicated by words in red).}
    \label{fig:spatial-gqa-multi-hop}
\end{figure}

==> tables/multihop_cot.tex <==
\begin{table}
    \centering
    \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{l|l|l|l|l}
    \hline
Model  & GPT-4o & GPT-4 vison & Gemini-Pro & LLaVA-1.5 \\\hline
     stan& 60.78& 50.65&43.18 &42.05\\
     stan+COT& 56.91 & 54.53& 45.39&39.91\\
     stan+bbox$_{\text{synth}}$&58.89 & 56.72&44.75 &46.14\\
     stan+SG$_{\text{synth}}$& \textbf{63.27}&  \textbf{66.00} &\textbf{60.35} &\textbf{54.90}\\
    \end{tabular}}
    \caption{We evaluated the accuracy of Standard, Chain-of-Thought (CoT), and our methods using synthesized bounding boxes (bbox$_{\text{synth}}$) and scene graphs (SG$_{\text{synth}}$) on the challenging multi-hop benchmark, Spatial-MM-Multi-hop. The best results within each dataset are highlighted in bold.}
    \label{tab:spatial-mm-multihop}
\end{table}







==> tables/prepositions.tex <==
\begin{table*}[]
\centering
\resizebox{0.99\linewidth}{!}{
\begin{tabular}{l|llll|llll}
\hline
Dataset & \multicolumn{4}{c}{GQA-spatial\_one\_obj}   & \multicolumn{4}{c}{GQA-spatial\_two\_obj}   \\\hline
Prepositions & total & front\_behind & left\_right & top\_bottom & total & front\_behind & left\_right & top\_bottom \\\hline
count  & 1160   & 2& 768   & 390   & 291 & 24   & 264   & 3 \\ \hline
Gmini (stan)& 18.60   & 0.0 & 19.45  & 17.01  & 18.21 & 25.00& 17.42   & 33.33   \\
Gmini (stan+bbox)   & 33.74   & 50.00 & 38.90  & 23.45  & 37.84   & 29.16& 38.31  & 66.67  \\
Gmini (stan+SG)  & \textbf{41.36}   & 0.0 & 45.75  & 32.81  & 60.07   & 70.83& 58.62  & 100   \\
Gmini (stan+SG+bbox) & 40.22   & 50.00 & 44.52  & 31.70  & 44.10   & 58.33& 42.91  & 33.33  \\ \hline
GPT4\_v (stan) & \_  & \_   & \_& \_& 23.71   & 79.16& 18.18  & 66.66  \\
GPT4\_v (stan+bbox) & \_  & \_   & \_& \_& 40.89   & 54.16& 39.39  & 66.67  \\
GPT4\_v (stan+SG)   & \_  & \_   & \_& \_& \textbf{76.63}   & 95.83& 74.62  & 100   \\ \hline
LLaVA (stan)& 32.33 & 0.0 & 38.67   & 20.00   & 18.56 & 20.83  & 18.18   & 33.33  \\
LLaVA (stan+bbox)  & 34.48 & 0.0  & 40.49   & 22.82  & 14.78 & 25.00   & 13.64 & 33.33 \\
LLaVA (stan+SG)  & 47.00 &34.00  &   &  &  &   &  & \\
LLaVA (stan+SG+bbox)  &  &  &   &  &  &   &  & \\
\hline 
\end{tabular}}
\end{table*}

==> tables/spatial_mm.tex <==
\begin{table}[]
\resizebox{0.99\linewidth}{!}{
\begin{tabular}{l|lll}
    \hline
    Model  & Spatial-MM-yes/no & Spatial-MM-others & Avg \\\hline
    GPT-4V  &   &    & \textbf{ }  \\
    Gemini-Pro &   &    &   \\
    LLaVA-1.5  &    &   &   \\
    mPLUG-Owl2 &    &    &  \\\hline
    Human & & &  \\
    Random Guess & 50& 25& 34\\\hline
\end{tabular}}
\caption{Results of zero-shot evaluation of varied multimodal LLMs on our benchmarks. All models perform poorly on spatial relations.}
\label{tab:spa_mm}
\end{table}
